Spectral Geometry for Deep Learning: Compression and Hallucination Detection via Random Matrix Theory

Large language models and deep neural networks achieve strong performance but suffer from reliability issues and high computational cost. This thesis proposes a unified framework based on spectral geometry and random matrix theory to address both problems by analyzing the eigenvalue structure of hidden activations. The first contribution, EigenTrack, is a real-time method for detecting hallucinations and out-of-distribution behavior in language and vision-language models using spectral features and their temporal dynamics. The second contribution, RMT-KD, is a principled compression method that identifies informative spectral components and applies iterative knowledge distillation to produce compact and efficient models while preserving accuracy. Together, these results show that spectral statistics provide interpretable and robust signals for monitoring uncertainty and guiding compression in large-scale neural networks.

==> sections/4_methodology/unified.tex <==
\section{Spectral Geometry for Reliable and Efficient Deep Learning}
\label{conclusion:unified_spectral_geometry}

The studies presented in this thesis demonstrate that spectral geometry and Random Matrix Theory provide a unifying foundation for both the reliability and efficiency of modern large-scale neural networks. Although EigenTrack and RMT-KD address distinct challenges, hallucination and out-of-distribution detection on one side, and compression and efficiency on the other, they emerge from the same mathematical insight: the eigenvalue spectrum of hidden activations encodes a compact, interpretable summary of model behavior. Through the spectral decomposition of covariance structures, it becomes possible to distinguish structured, causal representations from random noise, offering both diagnostic and constructive perspectives on deep learning dynamics.

In EigenTrack, temporal deviations from the Marchenko–Pastur law reveal early signs of instability, enabling proactive detection of hallucination and domain drift in large language and vision–language models. In RMT-KD, the same spectral principles identify the causal subspaces that carry informative structure, allowing principled dimensionality reduction without sacrificing accuracy. Together, these results show that the spectral manifold of activations acts as a shared space in which reliability and efficiency can be jointly optimized. This establishes Random Matrix Theory not merely as an analytical tool, but as a design principle for the next generation of interpretable, trustworthy, and energy-efficient artificial intelligence systems.

Beyond their immediate contributions, these findings suggest a broader research direction: spectral geometry can bridge the gap between statistical physics and deep learning, offering quantitative descriptors of representation quality and stability that generalize across modalities. The same framework that detects failure can also guide adaptation, calibration, and self-compression of models at scale. As model sizes continue to grow, this dual capability, to understand when networks fail and how to make them more compact, will be central to building reliable and sustainable AI systems.
